Variational Sequential Monte Carlo

Many recent advances in large scale probabilistic inference rely on variational methods. The success of variational approaches depends on (i) formulating a flexible parametric family of distributions, and (ii) optimizing the parameters to find the member of this family that most closely approximates the exact posterior. In this paper we present a new approximating family of distributions, the variational sequential Monte Carlo (VSMC) family, and show how to optimize it in variational inference. VSMC melds variational inference (VI) and sequential Monte Carlo (SMC), providing practitioners with flexible, accurate, and powerful Bayesian inference. The VSMC family is a variational family that can approximate the posterior arbitrarily well, while still allowing for efficient optimization of its parameters. We demonstrate its utility on state space models, stochastic volatility models for financial data, and deep Markov models of brain neural circuits.

==> preamble.tex <==
% to compile a camera-ready version, add the [final] option, e.g.:
% \usepackage[final]{nips_2016}

% For citations
\usepackage{natbib}

\usepackage[accepted]{aistats2018}

% use Times
\usepackage{times}
\RequirePackage{xspace} 
% For figures
\usepackage{graphicx} % more modern
%\usepackage{epsfig} % less modern
\usepackage{subcaption}
%\usepackage{subfigure} 
\usepackage{wrapfig}
% For tables
\usepackage{multirow}
\usepackage{hhline}

% For algorithms
\usepackage{algorithm}
\usepackage{algorithmic}

\usepackage{enumerate}
\usepackage[inline]{enumitem}
\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts

\usepackage[usenames,dvipsnames]{xcolor}
\definecolor{shadecolor}{gray}{0.9}

\newcommand{\red}[1]{\textcolor{BrickRed}{#1}}
\newcommand{\orange}[1]{\textcolor{BurntOrange}{#1}}
\newcommand{\green}[1]{\textcolor{OliveGreen}{#1}}

\newcommand{\blue}[1]{\textcolor{MidnightBlue}{#1}}
\newcommand{\gray}[1]{\textcolor{black!60}{#1}}
\newcommand{\lightgray}[1]{\textcolor{black!80}{#1}}

\usepackage[colorlinks,linktoc=all]{hyperref}
\usepackage[all]{hypcap}
\hypersetup{citecolor=MidnightBlue}
\hypersetup{urlcolor=MidnightBlue}
\hypersetup{linkcolor=Black}

\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
\usepackage{lipsum}
\usepackage{array}

% Packages hyperref and algorithmic misbehave sometimes.  We can fix
% this with the following command.
\newcommand{\theHalgorithm}{\arabic{algorithm}}

% Math
\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{amsthm}
\usepackage{amssymb}
\newtheorem{theorem}{Theorem}
\newtheorem{prop}{Proposition}

% Abbreviations
% Acronyms
\usepackage[acronym,smallcaps,nowarn]{glossaries}
\input{preamble_acronyms}
\newcommand{\ie}{i.e.\@\xspace}
\newcommand{\eg}{e.g.\@\xspace}

% Notation
\newcommand{\g}{\, ;}
\newcommand{\E}{\mathbb{E}}
\newcommand{\var}{\ensuremath{\operatorname{Var}}}
\newcommand{\eps}{\varepsilon}
\newcommand{\tL}{\tilde{\mathcal{L}}}
\newcommand{\prb}{\Pr}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\myd}{\mathrm{d}}
\newcommand{\given}{\,|\,}

\usepackage[color=yellow]{todonotes}


==> preamble_acronyms.tex <==
% A
\newacronym{ADVI}{advi}{automatic differentiation variational inference}

% B
\newacronym{BBVI}{bbvi}{black-box variational inference}
\newacronym{BPF}{bpf}{bootstrap particle filter}

% C
\newacronym{CTM}{ctm}{correlated topic model}

% D
\newacronym[\glslongpluralkey={deep exponential families}]{DEF}{def}{deep exponential family}
\newacronym{DMIS}{dmis}{deterministic multiple importance sampling}

% E
\newacronym{ELBO}{elbo}{evidence lower bound}

% G
\newacronym{GNTS}{gn-ts}{gamma-normal time series model}
\newacronym{G-REP}{g-rep}{generalized reparameterization}

% K
\newacronym{KL}{kl}{{K}ullback-{L}eibler}

% L
\newacronym{LDA}{lda}{latent {D}irichlet allocation}

% M
\newacronym{MF}{mf}{matrix factorization}
\newacronym{MIS}{mis}{multiple importance sampling}
\newacronym{MATLAB}{matlab}{MATLAB}

% N
\newacronym{NIPS}{nips}{Neural Information Processing Systems}
\newacronym{NLM}{nlm}{Narendra-Li model}

% O
\newacronym{OBBVI}{o-bbvi}{overdispersed black-box variational inference}

% R
\newacronym{RS-VI}{rsvi}{rejection sampling variational inference}

% S
\newacronym{SVI}{svi}{stochastic variational inference}
\newacronym{SMC}{smc}{sequential Monte Carlo}
\newacronym{SNR}{snr}{signal-to-noise ratio}
\newacronym{SSM}{ssm}{state space model}

% V
\newacronym{VI}{vi}{variational inference}
\newacronym{VIS}{vis}{variational importance sampling}
\newacronym{VB}{vb}{variational Bayes}
\newacronym{VEM}{vem}{variational expectation-maximization}
\newacronym{VSMC}{vsmc}{variational sequential Monte Carlo}
\newacronym{IWAE}{iwae}{importance weighted auto-encoder}

